Liquidity takers behavior representation through a contrastive learning approach

Thanks to the access to the labeled orders on the CAC40 data from Euronext, we are able to analyze agents' behaviors in the market based on their placed orders. In this study, we construct a self-supervised learning model using triplet loss to effectively learn the representation of agent market orders. By acquiring this learned representation, various downstream tasks become feasible. In this work, we utilize the K-means clustering algorithm on the learned representation vectors of agent orders to identify distinct behavior types within each cluster.

==> triplet.tex <==
Triplet loss $\sum_i^N \max\big(||f(x_i^a)-f(x_i^p)||_2^2 - ||f(x_i^a)-f(x_i^n)||_2^2 + \gamma, 0\big)$
where 
\begin{itemize}
    \item $f$ is the embedding function
    \item $\gamma$ is a margin between positive and negative pairs
    \item $a$ indicates \textbf{Anchor} sample, $p$ indicates \textbf{Positive} sample, $n$ indicates \textbf{Negative} sample.
\end{itemize}
\begin{figure}[h]
    \centering
    \includegraphics[width=0.7\textwidth]{Chapter5/figures/triplet.png}
    \caption[Triplet Illustration]{Triplet Loss illustration. Image from \cite{schroff2015facenet}}
    \label{fig:triplet}
\end{figure}

\paragraph{Input} Input $x$ is a sequence of $50$ consecutive trade orders executed by one agent $\alpha$ (note this set as $\mathcal{X}_\alpha$). The triplet input consists of $x^a, x^p, x^n$ where $x^a$ and $x^p$ come from the same agent will $x^n$ comes from another agent, $x^a \neq x^p$. 
\begin{itemize}
    \item Local model : the triplet should be constructed locally. The time of the positive sample $x^p$ and the negative sample $x^n$ should be close the that of the anchor, for example no more than 2 hours. The "time" of a sample of 50 orders means the timestamp of the first order.
    
    The reason why we use the local model is that the agents can change their strategies over time. It is not natural if we force two inputs of an agent to match while they are very far from each other on time. In this case, we can benefit a lot from the contrastive model.
\end{itemize}
\paragraph{Embedding} $f(x) = LSTM(x)$
